Depth-conditioned Dynamic Message Propagation for Monocular 3D Object Detection

The objective of this paper is to learn context- and depth-aware feature representation to solve the problem of monocular 3D object detection. We make following contributions: (i) rather than appealing to the complicated pseudo-LiDAR based approach, we propose a depth-conditioned dynamic message propagation (DDMP) network to effectively integrate the multi-scale depth information with the image context;(ii) this is achieved by first adaptively sampling context-aware nodes in the image context and then dynamically predicting hybrid depth-dependent filter weights and affinity matrices for propagating information; (iii) by augmenting a center-aware depth encoding (CDE) task, our method successfully alleviates the inaccurate depth prior; (iv) we thoroughly demonstrate the effectiveness of our proposed approach and show state-of-the-art results among the monocular-based approaches on the KITTI benchmark dataset. Particularly, we rank $1^{st}$ in the highly competitive KITTI monocular 3D object detection track on the submission day (November 16th, 2020). Code and models are released at \url{https://github.com/fudan-zvg/DDMP}

==> table/table_architecture.tex <==
\begin{table*}[htp]
 \caption{Detailed architecture. The table expands the details of the DDMP process on image stage II (DDMP\_1), including the message propagation from image stage II and depth stage II / III / IV, and the message updating on image stage II.}
 \small
 \centering
 \begin{tabular}{|c|c|c|c|}
  \hline
  Module & Type / Stride &    Input name &  Output name: size                         \\
  \hline
  \hline
  \multirow{5}*{Detection backbone (ResNet-50)} 
  &   conv1 / s=2 &   image 
  &  img\_conv1:  $64 \times 256 \times 880$ \\
  &   conv2\_x / s=2 &  img\_conv1
  &  img\_stage1:  $256 \times 128 \times 440$ \\
  &   conv3\_x / s=2 &  img\_stage1
  &  img\_stage2:  $512 \times 64 \times 220$ \\
  &   conv4\_x / s=2 &  img\_stage2
  &  img\_stage3:  $1024 \times 32 \times 110$ \\
  &   conv5\_x (dilated=2) / s=1&  img\_stage3
   &  img\_stage4:  $2048 \times 32 \times 110$ \\
  \hline
  \hline
  \multirow{5}*{Depth backbone (ResNet-50)} 
  &   conv1 / s=2 &  estimated depth map
  &  dep\_conv1:  $64 \times 256 \times 880$ \\
  &   conv2\_x / s=2 &  dep\_conv1
  &  dep\_stage1:  $256 \times 128 \times 440$ \\
  &   conv3\_x / s=2 &  dep\_stage1
  &  dep\_stage2:  $512 \times 64 \times 220$ \\
  &   conv4\_x / s=2 &  dep\_stage2
  &  dep\_stage3:  $1024 \times 32 \times 110$ \\
  &   conv5\_x (dilated=2) / s=1&  dep\_stage3
   &  dep\_stage4:  $2048 \times 32 \times 110$ \\
  \hline
  \hline
  \multirow{10}*{DDMP\_1 (stage2\_depth2)}
  &   conv 1 \times 1 &  img\_stage2 
  &   img\_stage22: $256 \times 64 \times 220$ \\
  &   conv 3 \times 3 &  img\_stage22 
  &   img\_stage22\_offset: $18 \times 64 \times 220$ \\
  &   deform\_unfold 3 \times 3 &  img\_stage22 
  &   img\_stage22\_sample: $256 \times 9 \times 64 \times 220$ \\
  &   conv 1 \times 1 &  dep\_stage2 
  &   dep\_stage22: $256 \times 64 \times 220$ \\
  &   deform\_conv 3 \times 3 (group=1) &  dep\_stage22 
  &   dep\_stage22\_affinity: $9 \times 64 \times 220$ \\
  &   conv 3 \times 3 &  dep\_stage22 
  &   dep\_stage22\_filter: $9 \times 64 \times 220$ \\
  &   \multirow{2}*{dot} &  img\_stage22\_sample;& \multirow{2}*{stage22\_sample: $256 \times 9 \times (64 * 220)$ }\\
  && dep\_stage22\_filter &   \\
  &   \multirow{2}*{matmul(group=1)} &  stage22\_sample;& \multirow{2}*{message\_stage22: $256 \times 64 \times 220$ }\\
  && dep\_stage22\_affinity &   \\
  
  \hline
  \multirow{2}*{DDMP\_1 (stage2\_depth3)}&   
  Similar to stage2\_depth2 &  img\_stage2;& \multirow{2}*{message\_stage23: $256 \times 64 \times 220$ }\\
  &(+ interpolate on dep\_stage3)& dep\_stage3 &   \\
  \hline
  \multirow{2}*{DDMP\_1 (stage2\_depth4)}&   
  Similar to stage2\_depth2 &  img\_stage2;& \multirow{2}*{message\_stage24: $256 \times 64 \times 220$ }\\
  &(+ interpolate on dep\_stage4)& dep\_stage4 &   \\
  \hline
  DDMP\_1 (update)&   
  \multirow{2}*{concat \& conv 3 \times 3} &  img\_stage2;& \multirow{2}*{img\_stage2: $512 \times 64 \times 220$ }\\
  && message\_stage22/23/24 &   \\
  \hline
  \multirow{2}*{DDMP\_2}&   
  \multirow{2}*{Similar to DDMP\_1} &  img\_stage3;& \multirow{2}*{img\_stage3: $1024 \times 32 \times 110$ }\\
  && dep\_stage2/3/4 &   \\
  \hline
  
  \hline
 \end{tabular}
 \label{tab_arch}
\end{table*}

